A Survey on Point-of-Interest Recommendation: Models, Architectures, and Security

The widespread adoption of smartphones and Location-Based Social Networks has led to a massive influx of spatio-temporal data, creating unparalleled opportunities for enhancing Point-of-Interest (POI) recommendation systems. These advanced POI systems are crucial for enriching user experiences, enabling personalized interactions, and optimizing decision-making processes in the digital landscape. However, existing surveys tend to focus on traditional approaches and few of them delve into cutting-edge developments, emerging architectures, as well as security considerations in POI recommendations. To address this gap, our survey stands out by offering a comprehensive, up-to-date review of POI recommendation systems, covering advancements in models, architectures, and security aspects. We systematically examine the transition from traditional models to advanced techniques such as large language models. Additionally, we explore the architectural evolution from centralized to decentralized and federated learning systems, highlighting the improvements in scalability and privacy. Furthermore, we address the increasing importance of security, examining potential vulnerabilities and privacy-preserving approaches. Our taxonomy provides a structured overview of the current state of POI recommendation, while we also identify promising directions for future research in this rapidly advancing field.

==> abstract.tex <==

\begin{abstract}
The widespread adoption of smartphones and Location-Based Social Networks has led to a massive influx of spatio-temporal data, creating unparalleled opportunities for enhancing Point-of-Interest (POI) recommendation systems. These advanced POI systems are crucial for enriching user experiences, enabling personalized interactions, and optimizing decision-making processes in the digital landscape. However, existing surveys tend to focus on traditional approaches and few of them delve into cutting-edge developments, emerging architectures, as well as security considerations in POI recommendations. To address this gap, our survey stands out by offering a comprehensive, up-to-date review of POI recommendation systems, covering advancements in models, architectures, and security aspects. We systematically examine the transition from traditional models to advanced techniques such as large language models. Additionally, we explore the architectural evolution from centralized to decentralized and federated learning systems, highlighting the improvements in scalability and privacy. Furthermore, we address the increasing importance of security, examining potential vulnerabilities and privacy-preserving approaches. Our taxonomy provides a structured overview of the current state of POI recommendation, while we also identify promising directions for future research in this rapidly advancing field.
\end{abstract}



==> data.tex <==

% \section{Dataset Description}
% \label{sec:data}

The NYC Restaurant Rich Dataset~\cite{yang2013fine,yang2013sentiment} provides detailed check-in, tip, and tag data for New York restaurants, useful for studying location recommendations and user preferences. The NYC and Tokyo Check-in Dataset~\cite{yang2014modeling} covers nearly 10 months of check-ins from these cities, focusing on spatial-temporal activity patterns. The Global-scale Check-in Dataset~\cite{yang2015nationtelescope} expands this scope to 77 countries, offering a broader view of collective behaviors and social interactions. The User Profile Dataset~\cite{yang2016privcheck} offers anonymized user profiles from New York and Tokyo, contributing to privacy-related studies. Lastly, the Global-scale Check-in Dataset~\cite{yang2019revisiting} with User Social Networks includes social network snapshots and extends the global check-in data, facilitating research into social interactions and mobility patterns across diverse regions.



















% The NYC Restaurant Rich Dataset~\cite{yang2013fine,yang2013sentiment,yang2014sesame} provides detailed check-in, tip, and tag data for New York restaurants, useful for studying location recommendations and user preferences. The NYC and Tokyo Check-in Dataset~\cite{yang2014modeling} covers nearly 10 months of check-ins from these cities, focusing on spatial-temporal activity patterns. The Global-scale Check-in Dataset~\cite{yang2015nationtelescope,yang2016participatory} expands this scope to 77 countries, offering a broader view of collective behaviors and social interactions. The User Profile Dataset~\cite{yang2016privcheck,yang2018privacy} offers anonymized user profiles from New York and Tokyo, contributing to privacy-related studies. Lastly, the Global-scale Check-in Dataset~\cite{yang2019revisiting,yang2020lbsn2vec++} with User Social Networks includes social network snapshots and extends the global check-in data, facilitating research into social interactions and mobility patterns across diverse regions.

% \subsection{Foursquare Dataset}

% The Foursquare dataset\footnote{https://sites.google.com/site/yangdingqi/home/foursquare-dataset} provides extensive check-in data alongside user social network information from multiple LBSNs. This dataset has been widely used in research on personalized location recommendations and search functionalities. It consists of five subsets: the New York City Restaurant Rich Dataset, NYC and Tokyo Check-in Dataset, Global-scale Check-in Dataset, User Profile Dataset, and Global-scale Check-in Dataset with User Social Networks. These subsets include data from locations such as New York City (NYC), Tokyo (TKY), and Charlotte (CHA).

% The NYC Restaurant Rich Dataset~\cite{yang2013fine,yang2013sentiment,yang2014sesame} provides detailed check-in, tip, and tag data for New York restaurants, useful for studying location recommendations and user preferences. The NYC and Tokyo Check-in Dataset~\cite{yang2014modeling} covers nearly 10 months of check-ins from these cities, focusing on spatial-temporal activity patterns. The Global-scale Check-in Dataset~\cite{yang2015nationtelescope,yang2016participatory} expands this scope to 77 countries, offering a broader view of collective behaviors and social interactions. The User Profile Dataset~\cite{yang2016privcheck,yang2018privacy} offers anonymized user profiles from New York and Tokyo, contributing to privacy-related studies. Lastly, the Global-scale Check-in Dataset~\cite{yang2019revisiting,yang2020lbsn2vec++} with User Social Networks includes social network snapshots and extends the global check-in data, facilitating research into social interactions and mobility patterns across diverse regions.


% \textbf{NYC Restaurant Rich Dataset}~\cite{yang2013fine,yang2013sentiment,yang2014sesame}. This dataset comprises check-in, tip, and tag data from restaurant venues in New York City, collected between October 24, 2011, and February 20, 2012. It includes 3,112 users and 3,298 venues, with a total of 27,149 check-ins and 10,377 tips. This dataset is a highly valuable resource for studying personalized location recommendations, search problems, user behavior patterns, and geographic preferences across diverse populations and environments.

% \textbf{NYC and Tokyo Check-in Dataset}~\cite{yang2014modeling}. This dataset contains check-in data collected over approximately ten months, from April 12, 2012, to February 16, 2013, in New York City and Tokyo. It includes 227,428 check-ins from New York City and 573,703 check-ins from Tokyo, with each record providing a timestamp, GPS coordinates, and detailed venue categories. This dataset is primarily used to analyze the spatial-temporal patterns of user activities in LBSNs.

% \textbf{Global-scale Check-in Dataset}~\cite{yang2015nationtelescope,yang2016participatory}. This global dataset, spanning from April 2012 to September 2013, covers 415 cities across 77 countries. It includes 33,278,683 check-ins by 266,909 users at 3,680,126 venues. This dataset is particularly valuable for large-scale studies on collective behavior, as it offers a comprehensive and detailed source of information that enables researchers to explore patterns of group dynamics, decision-making, and social interactions across diverse contexts.

% \textbf{User Profile Dataset}~\cite{yang2016privcheck,yang2018privacy}. This dataset provides basic user profile information, such as gender, number of friends, and number of followers, specifically for privacy studies. It includes data from 18,201 users in New York City and 11,874 users in Tokyo. Anonymized user IDs allow this dataset to be linked with the global-scale check-in dataset, offering crucial data for research focused on privacy issues.

% \textbf{Global-scale Check-in Dataset with User Social Networks}~\cite{yang2019revisiting,yang2020lbsn2vec++}. This dataset extends the global-scale check-in dataset by including user social network data. It spans 22 months, from April 2012 to January 2014, and includes two snapshots of user social networks before and after the check-in data collection period. The dataset contains 22,809,624 check-ins along with information on 363,704 old and 607,333 new friendships. Additionally, it offers a raw check-in dataset comprising 90,048,627 check-ins by 2,733,324 users at 11,180,160 venues, providing rich and diverse data for studying user mobility patterns and social interactions within LBSNs across various regions and contexts.


\subsection{Gowalla Dataset}

Gowalla is a location-based social network where users shared their locations via check-ins. The Gowalla dataset\footnote{http://snap.stanford.edu/data/loc-gowalla.html} contains check-in data from users in California and Nevada, spanning February 2009 to October 2010. It includes 6,442,890 check-in entries from 10,162 users across 24,250 POIs.

This dataset also features an undirected social network comprising 196,591 nodes and 950,327 edges. The network is fully connected, with an average clustering coefficient of 0.2367, containing 2,273,138 triangles and a network diameter of 14. The 90-percentile effective diameter is 5.7, indicating that most nodes are accessible within a few steps~\cite{cho2011friendship}.

\subsection{Brightkite Dataset}

Brightkite is a location-based social network where users could check in to share locations and connect with friends. The Brightkite dataset\footnote{http://snap.stanford.edu/data/loc-brightkite.html} contains global check-in data spanning May 2008 to October 2010, with 4,491,143 check-ins by 1,850 users across 1,672 POIs, offering insights into user mobility, social interactions, and location preferences. Additionally, the dataset includes a directed social network with 58,228 nodes and 214,078 edges, which can be simplified to an undirected network by considering only bi-directional edges~\cite{cho2011friendship}.

\subsection{Yelp Dataset}

Yelp is a popular platform where users rate and review businesses, has featured listings from major cities across more than 20 countries since 2005. The Yelp dataset\footnote{https://www.yelp.com/dataset} offers valuable real-world data for research, including 6,990,280 reviews, 150,346 businesses, 200,100 pictures, and data from 11 metropolitan areas. It also includes over 908,915 tips from 1,987,897 users, business attributes for 1.2 million businesses, and aggregated check-in data for 131,930 businesses. The dataset is organized into six tables—Business, Reviews, Users, Checkin, Tip, and Photo—providing a comprehensive view of user-business interactions for analysis.

\subsection{Weeplaces Dataset}

Weeplaces is a service that visually mapped user check-ins across various location-based platforms. Now integrated with APIs from services like Facebook Places, Foursquare, and Gowalla, Weeplaces allowed users to log in with their LBSN accounts and connect with friends. The Weeplaces dataset\footnote{http://www.yongliu.org/datasets} contains 7,658,368 check-ins from 15,799 users across 971,309 locations. Although the original Foursquare IDs are unavailable, the dataset provides check-in history, friend connections, and additional location information.

\subsection{Other Datasets}

A variety of datasets have been collected from social media platforms such as Twitter, Instagram, Facebook, WeChat, Douban, and Baidu Maps~\cite{islam2022survey}. Twitter provides location data through user status updates and check-ins, accessible via its public API. Instagram focuses on photo and video sharing, allowing users to browse content by tags and geographic locations. Its dataset, containing user check-ins, is frequently used in POI recommendation research. Facebook, the world’s largest social media platform, offers diverse media sharing, including check-in data, making it valuable for POI prediction. WeChat includes messaging, video calls, and location sharing, while Douban facilitates organizing offline social events with online check-ins. Baidu Maps provides tools like street maps, satellite imagery, and route planning.

% \textbf{Summary}. The datasets discussed above typically contain user-POI data, including check-in details such as timestamps, locations, and semantic features. POI semantic data includes categories, tags from user posts, creation dates, geolocations, check-in counts, user numbers, and radii. User semantic features encompass posts, friends, and check-ins. Additionally, datasets like Foursquare, Gowalla, and Weeplaces include user-user relationships, structured in a many-to-many format connecting users to their friends. Due to the vast data volume and check-in numbers, some of these datasets are quite large, prompting much research to focus on specific regions for effective data management.



























==> model.tex <==
\section{Preliminary} 
























==> relate.tex <==
\section{Related Surveys}
\label{sec:related}

{\color{red}{
only compare POI recommendation survey, emphasize our contributions, skip the section of related survey.
}}




% Within the spatio-temporal domain, existing surveys can be broadly classified into two main categories: spatio-temporal data mining and spatio-temporal forecasting. Surveys focusing on spatio-temporal data mining, such as those conducted by Zhang \textit{et al.}\cite{zhang2024survey}, Wang \textit{et al.}\cite{wang2020deep}, Atluri \textit{et al.}\cite{atluri2018spatio}, Alam \textit{et al.}\cite{alam2022survey}, and Yuan \textit{et al.}\cite{yuan2021survey}, emphasize generative techniques or deep learning methodologies for analyzing spatio-temporal data. For instance, Zhang \textit{et al.}\cite{zhang2024survey} offer a comprehensive overview of techniques like Seq2seq, self-supervised learning, Large Language Models (LLMs) including models such as BERT~\cite{devlin2019bert} and GPT-3~\cite{radford2019language}, and Denoising Diffusion Probabilistic Models (DDPMs)\cite{ho2020denoising}. Notably, these surveys do not delve into foundational models like Mamba\cite{gu2023mamba} or deep learning methods specifically tailored for Point of Interest (POI) recommendation. On the other hand, surveys focusing on spatio-temporal forecasting, exemplified by works such as those by Bui \textit{et al.}\cite{bui2022spatial}, Luo \textit{et al.}\cite{luo2021spatial}, and Tascikaraoglu \textit{et al.}\cite{tascikaraoglu2018evaluation}, concentrate on predicting future values of spatio-temporal data. While these surveys encompass a range of forecasting techniques, they do not explicitly address foundational models or deep learning methods relevant to POI recommendation. For instance, Bui \textit{et al.}\cite{bui2022spatial} emphasize an extensive overview of traffic prediction, rather than POI recommendation. Moreover, an earlier work by Tascikaraoglu \textit{et al.}~\cite{tascikaraoglu2018evaluation} provides a comprehensive examination of existing spatio-temporal methods, including deep learning techniques, but does not focus on POI recommendation, lacking a detailed exploration of models, architectures, and security considerations within this specific context.
In the domain of spatio-temporal data analysis, surveys are typically bifurcated into two principal categories: spatio-temporal data mining and spatio-temporal forecasting. Surveys in the spatio-temporal data mining domain, such as those conducted by Zhang et al. \cite{zhang2024survey}, Wang et al. \cite{wang2020deep}, Atluri et al. \cite{atluri2018spatio}, Alam et al. \cite{alam2022survey}, and Yuan et al. \cite{yuan2021survey}, prominently highlight generative techniques and deep learning methodologies tailored for analyzing spatio-temporal data. For instance, Zhang et al. provide an extensive overview of techniques like Seq2seq, self-supervised learning, Large Language Models (LLMs) encompassing models such as BERT and GPT-3, and Denoising Diffusion Probabilistic Models (DDPMs). However, these surveys often lack in-depth discussions on architecure and security explicitly designed for Point of Interest (POI) recommendation.


Conversely, surveys focusing on spatio-temporal forecasting, as exemplified by the works of Bui et al. \cite{bui2022spatial}, Luo et al. \cite{luo2021spatial}, and Tascikaraoglu et al. \cite{tascikaraoglu2018evaluation}, primarily center on predicting future values within spatio-temporal datasets. While these surveys encompass a diverse array of forecasting techniques, they often sideline fundamental models or deep learning strategies relevant to POI recommendation. For instance, Bui et al. provide an extensive review of traffic prediction rather than concentrating on POI recommendation. Similarly, the earlier work by Tascikaraoglu et al. offers a comprehensive examination of existing spatio-temporal methods, integrating deep learning techniques, but lacks a specific emphasis on POI recommendation, thus missing a detailed exploration of models, architectures, and security considerations within this unique context. This distinction underscores the pressing need for comprehensive surveys that bridge the gap between spatio-temporal data mining and forecasting, amalgamating insights to advance the understanding and development of POI recommendation systems amidst the intricate spatio-temporal landscape.



A specialized research domain~\cite{jitkajornwanich2020survey,pant2018survey,nandal2013spatio,alam2022survey} is dedicated to spatial-temporal databases, deviating from the realms of spatial-temporal prediction and spatial-temporal data mining previously discussed. While aligned in the objective of exploring spatial-temporal databases, this line of research sets itself apart by concentrating on contemporary traditional methodologies for spatio-temporal databases and the management of spatial-temporal data. It specifically investigates the utilization of deep learning or conventional techniques within the sphere of spatial-temporal databases, a scope that falls outside the purview of our present study on POI recommendation.





\textbf{Motivations of This Survey.} While existing surveys have explored Point of Interest (POI) recommendation, a gap persists in examining models, architectures, and security aspects within this domain, as illustrated in Table~\ref{tab:survey}. Notably, Zhao \textit{et al.} \cite{zhao2016survey} and Yu \textit{et al.} \cite{yu2015survey} have primarily focused on traditional methods like matrix factorization (MF)-based techniques \cite{li2009relation, lian2014geomf}. In contrast, Islam's survey \cite{islam2022survey} emphasizes deep learning methods for POI recommendation but overlooks architectural and security considerations. Furthermore, Werneck's earlier survey \cite{werneck2020survey} concentrates on methods for POI recommendation between 2017 and 2019. This study endeavors to bridge this gap by delivering a comprehensive and current overview of models, architectures, and security measures relevant to POI recommendation. It also introduces a detailed taxonomy to enhance understanding of the field. By amalgamating insights from previous research and exploring uncharted territories, this survey aspires to provide a holistic perspective on the evolving landscape of POI recommendation systems. Through this holistic analysis, we aim to contribute to the advancement and refinement of POI recommendation methodologies, ensuring that future systems are not only efficient and accurate but also robust, secure, and adaptable to emerging technological trends.








